Homophily in preferences or meetings? Identifying and estimating an iterative network formation model

Is homophily in social and economic networks driven by a taste for homogeneity (preferences) or by a higher probability of meeting individuals with similar attributes (opportunity)? This paper studies identification and estimation of an iterative network game that distinguishes between these two mechanisms. Our approach enables us to assess the counterfactual effects of changing the meeting protocol between agents. As an application, we study the role of preferences and meetings in shaping classroom friendship networks in Brazil. In a network structure in which homophily due to preferences is stronger than homophily due to meeting opportunities, tracking students may improve welfare. Still, the relative benefit of this policy diminishes over the school semester.

==> tables/coefs_postlasso_trim_FALSE.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Thu Apr 22 21:46:40 2021
\begin{table}[H]
\centering
\caption{Posterior estimates - Post-lasso summary statistics method} 
\begin{tabular}{lllll}
  \hline
  & Mean & Q 0.025 & Q 0.975 & Prob $<$ 0 \\ 
  \hline \multicolumn{5}{c}{ Meeting process } \\ \hline  \hline
distance in age &  1.4032 & -3.2346 &  3.3159 &  0.2829 \\ 
  distance in gender &  0.2589 & -1.6056 &  2.6820 &  0.1715 \\ 
  distance in cognitive skills &  2.0731 & -1.0589 &  3.7073 &  0.1495 \\ 
  distance in conscientiousness & -1.0811 & -2.8893 &  3.7171 &  0.8296 \\ 
  distance in neuroticism &  0.4306 & -3.3669 &  3.2945 &  0.2860 \\ 
  g\_ij &  3.0958 & -1.7662 &  4.6653 &  0.1146 \\ 
  (1-g\_ij)*distance in classlist & -0.9584 & -4.1177 &  1.4827 &  0.8462 \\ 
   \hline \multicolumn{5}{c}{ Utility -- Direct Links } \\ \hline intercept & -0.1782 & -2.6117 &  1.0531 &  0.7561 \\ 
  distance in age & -1.8191 & -3.5752 & -0.1818 &  0.9815 \\ 
  distance in gender & -2.6171 & -5.0266 &  0.2951 &  0.9211 \\ 
  distance in cognitive skills &  1.0173 & -2.8939 &  2.9317 &  0.1827 \\ 
  distance in conscientiousness & -0.1933 & -3.0842 &  0.9110 &  0.4049 \\ 
  distance in neuroticism &  1.1115 & -3.5467 &  2.3263 &  0.2003 \\ 
   \hline \multicolumn{5}{c}{ Utility -- Reciprocity Links } \\ \hline intercept &  1.6716 &  0.3899 &  4.4766 &  0.0175 \\ 
  distance in age & -0.1104 & -3.8150 &  1.9351 &  0.2630 \\ 
  distance in gender & -0.1749 & -3.7851 &  1.9078 &  0.3272 \\ 
  distance in cognitive skills &  1.1116 & -2.8162 &  4.2491 &  0.2047 \\ 
  distance in conscientiousness &  1.4742 &  0.2475 &  4.8784 &  0.0141 \\ 
  distance in neuroticism &  1.0765 & -0.8991 &  3.4033 &  0.0798 \\ 
   \hline \multicolumn{5}{c}{ Utility -- Indirect/Popularity } \\ \hline intercept &  1.3990 & -0.5646 &  2.2734 &  0.0559 \\ 
  distance in age & -2.7439 & -3.8436 & -0.6725 &  0.9890 \\ 
  distance in gender & -1.8800 & -4.3897 & -0.0880 &  0.9847 \\ 
  distance in cognitive skills &  1.0723 & -1.2559 &  3.1169 &  0.1848 \\ 
  distance in conscientiousness & -1.8519 & -3.2410 &  0.2173 &  0.9687 \\ 
  distance in neuroticism & -0.0830 & -2.1986 &  1.0819 &  0.2418 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/ols_counter_unweighted_acceptance_0.01.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Jan 22 03:19:15 2020
\begin{table}[H]
\centering
\caption{Homophily measures under base counterfactual policies. Unweighted criterion. Acceptance rate: 0.01. $\hat{\tau}_0 = 76$.}
\label{ols_counter_unweighted_acceptance_0.01}
\begin{adjustbox}{width = \textwidth}
\begin{tabular}{cccc}
  \hline & base & random & tracking \\ 
  \hline
distance in classlist & -0.0068 & -0.0016 & -0.0124 \\ 
   & [-0.009;-0.0037] & [-0.0023;-6e-04] & [-0.0155;-0.0089] \\ 
  distance in age & -0.0146 & -0.0161 & -0.0152 \\ 
   & [-0.0183;-0.0097] & [-0.0214;-0.0109] & [-0.0236;-0.0053] \\ 
  distance in gender & -0.0921 & -0.1077 & -0.0421 \\ 
   & [-0.1042;-0.0791] & [-0.1197;-0.0993] & [-0.0532;-0.0335] \\ 
  distance in cognitive skills & -0.0955 & -0.1342 & 0.0322 \\ 
   & [-0.1448;-0.0514] & [-0.1952;-0.0809] & [-0.0426;0.0999] \\ 
  distance in conscientiousness & -0.0122 & -0.0117 & -0.0079 \\ 
   & [-0.0234;-0.0021] & [-0.0218;-0.0011] & [-0.0231;1e-04] \\ 
  distance in neuroticism & -0.0111 & -0.0106 & -0.0102 \\ 
   & [-0.0196;-0.0052] & [-0.0194;-0.0038] & [-0.0195;4e-04] \\ 
   \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/ols_counter_unweighted_acceptance_0_01_RF.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 19 17:17:15 2020
\begin{table}[H]
\centering
\caption{Homophily measures under base counterfactual policies. Unweighted criterion. Acceptance rate: 0.01. $\hat{\tau}_0 = 76$.} 
\label{ols_counter_unweighted_acceptance_0.05}
\begin{tabular}{ccccc}
  \hline
rows & base & random & tracking & noutility \\ 
  \hline
distance in classlist & -0.0052 & -0.0017 & -0.0109 & -0.0071 \\ 
   & [-0.0097;2e-04] & [-0.0025;-8e-04] & [-0.0173;-0.0047] & [-0.012;7e-04] \\ 
  distance in age & 9e-04 & 7e-04 & -0.0035 & 9e-04 \\ 
   & [-0.0154;0.0195] & [-0.0159;0.0198] & [-0.02;0.0154] & [-0.0077;0.0116] \\ 
  distance in gender & -0.103 & -0.1131 & -0.0464 & -0.0982 \\ 
   & [-0.1343;-0.0775] & [-0.14;-0.0882] & [-0.0716;-0.0234] & [-0.1166;-0.0832] \\ 
  distance in cognitive skills & -0.1094 & -0.1343 & 0.0293 & -0.124 \\ 
   & [-0.1694;-0.0467] & [-0.1935;-0.0736] & [-0.0762;0.1299] & [-0.1951;-0.0609] \\ 
  distance in conscientiousness & -0.0131 & -0.0141 & -0.0068 & -0.0084 \\ 
   & [-0.0351;0.0099] & [-0.0378;0.0102] & [-0.0283;0.0176] & [-0.0234;0.0079] \\ 
  distance in neuroticism & -0.0116 & -0.0123 & -0.0106 & -0.0091 \\ 
   & [-0.0317;0.0073] & [-0.0337;0.0084] & [-0.0322;0.0116] & [-0.0227;0.0049] \\ 
   \hline
\end{tabular}
\end{table}


==> tables/ols_postlasso_trim_FALSE.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Thu Apr 22 21:47:05 2021
\begin{table}[H]
\centering
\caption{Projection coefficients and edge statistics - Post-lasso summary statistics method} 
\begin{tabular}{llllll}
  \hline
  & Data & Base case & Random matching & Tracking & Random friendship \\ 
  \hline \multicolumn{4}{c}{ Regression coefficients } \\ \hline  \hline
distance in classlist & -0.0016 & -0.0005 & -0.0007 & -0.0005 &  0.0043 \\ 
    & [-0.0028;-0.0004] & [-0.0012; 0.0008] & [-0.0011; 0.0006] & [-0.0021; 0.0013] & [-0.0019; 0.0361] \\ 
  distance in age &  0.0018 & -0.0185 & -0.0246 & -0.0108 & -0.0147 \\ 
    & [-0.0048; 0.0083] & [-0.0324; 0.0150] & [-0.0322;-0.0043] & [-0.0197; 0.0056] & [-0.0897; 0.0243] \\ 
  distance in gender & -0.1864 & -0.0881 & -0.1769 & -0.0423 & -0.0632 \\ 
    & [-0.2072;-0.1657] & [-0.1856;-0.0239] & [-0.2228;-0.1188] & [-0.1051;-0.0120] & [-0.1562;-0.0105] \\ 
  distance in cognitive skills & -0.1275 & -0.0619 & -0.0838 &  0.0760 & -0.0770 \\ 
    & [-0.2172;-0.0378] & [-0.1360; 0.0356] & [-0.1477;-0.0325] & [-0.0127; 0.1754] & [-0.3409; 0.0148] \\ 
  distance in conscientiousness & -0.0193 &  0.0017 & -0.0174 &  0.0001 &  0.0050 \\ 
    & [-0.0332;-0.0053] & [-0.0369; 0.0438] & [-0.0473;-0.0029] & [-0.0372; 0.0214] & [-0.0598; 0.0954] \\ 
  distance in neuroticism & -0.0231 & -0.0013 &  0.0127 &  0.0032 & -0.0162 \\ 
    & [-0.0356;-0.0106] & [-0.0173; 0.0324] & [-0.0433; 0.0290] & [-0.0165; 0.0194] & [-0.0970; 0.0277] \\ 
   \hline \multicolumn{4}{c}{ Edge summary statistics } \\ \hline $\mathbb{E}[g_{ij}]$ & 0.1788 &  0.0711 &  0.1475 &  0.0371 &  0.1107 \\ 
    & [0.168;0.1896] & [0.0149;0.1791] & [0.1089;0.1628] & [0.0085;0.0968] & [0.0246;0.4314] \\ 
  $\operatorname{sd}[g_{ij}]$ & 0.3832 &  0.2425 &  0.3537 &  0.1802 &  0.2678 \\ 
    & [0.374;0.3921] & [0.1213;0.3834] & [0.3116;0.3692] & [0.0917;0.2956] & [0.1550;0.4953] \\ 
   \hline
\end{tabular}
\end{table}


==> tables/pred_RF.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Feb 17 20:46:54 2020
\begin{longtable}{cccc}
\caption{Random-forest approximation to posterior moments} \\ 
  \hline
  & Mean & Q .05 & Q.95 \\ 
  \hline \multicolumn{4}{c}{Matching parameters} \\ \hline
distance in age & 0.0289 & -0.1621 & 0.2189 \\ 
  distance in gender & -0.0178 & -0.2062 & 0.1866 \\ 
  distance in cognitive skills & -0.0045 & -0.2067 & 0.1914 \\ 
  distance in conscientiousness & 0.0125 & -0.204 & 0.1958 \\ 
  distance in neuroticism & -0.0032 & -0.1964 & 0.1972 \\ 
  g\_ij & 0.0286 & -0.1703 & 0.207 \\ 
  (1-g\_ij)*distance in classlist & -0.0689 & -0.2011 & 0.0686 \\ 
   \hline \multicolumn{4}{c}{Utility (direct links)} \\ \hline intercept & -0.0248 & -0.198 & 0.1768 \\ 
  distance in age & -0.013 & -0.2005 & 0.185 \\ 
  distance in gender & -0.0326 & -0.2296 & 0.1607 \\ 
  distance in cognitive skills & -0.012 & -0.2265 & 0.1906 \\ 
  distance in conscientiousness & -0.0163 & -0.2101 & 0.1797 \\ 
  distance in neuroticism & -0.0143 & -0.224 & 0.1726 \\ 
   \hline \multicolumn{4}{c}{Utility (reciprocal links)} \\ \hline intercept & -5e-04 & -0.2212 & 0.2109 \\ 
  distance in age & 0.0025 & -0.1978 & 0.1735 \\ 
  distance in gender & -0.0024 & -0.2035 & 0.222 \\ 
  distance in cognitive skills & 0.0051 & -0.2155 & 0.1932 \\ 
  distance in conscientiousness & -0.0046 & -0.1936 & 0.1921 \\ 
  distance in neuroticism & -0.0031 & -0.2092 & 0.2069 \\ 
   \hline \multicolumn{4}{c}{Utility (indirect links)} \\ \hline intercept & -0.0504 & -0.2368 & 0.1399 \\ 
  distance in age & -0.019 & -0.1815 & 0.1481 \\ 
  distance in gender & -0.0509 & -0.2247 & 0.1593 \\ 
  distance in cognitive skills & -0.0103 & -0.2176 & 0.1873 \\ 
  distance in conscientiousness & -0.0521 & -0.2146 & 0.1274 \\ 
  distance in neuroticism & -0.0359 & -0.2178 & 0.1398 \\ 
   \hline \multicolumn{4}{c}{Utility (popularity)} \\ \hline intercept & -0.0568 & -0.2254 & 0.1403 \\ 
  distance in age & -0.0153 & -0.1982 & 0.1472 \\ 
  distance in gender & -0.0573 & -0.2448 & 0.1401 \\ 
  distance in cognitive skills & -0.0058 & -0.2094 & 0.1911 \\ 
  distance in conscientiousness & -0.0396 & -0.2313 & 0.1297 \\ 
  distance in neuroticism & -0.042 & -0.2055 & 0.1441 \\ 
   \hline
\hline
\label{results_RF}
\end{longtable}


==> tables/results_RF.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 19 16:36:08 2020
\begin{longtable}{ccccc}
\caption{Posterior distribution. Unweighted criterion. Acceptance rate: 0.01. $\hat{\tau}_0 = 76$.} \\ 
  \hline
  & Mean & Q .05 & Q.95 & Prob $<$ 0 \\ 
  \hline \multicolumn{5}{c}{Matching parameters} \\ \hline
distance in age & 0.0304 & -0.1344 & 0.2115 & 0.3886 \\ 
  distance in gender & -0.0049 & -0.1746 & 0.1746 & 0.53 \\ 
  distance in cognitive skills & -6e-04 & -0.189 & 0.1775 & 0.4943 \\ 
  distance in conscientiousness & 0.0015 & -0.1827 & 0.1706 & 0.4986 \\ 
  distance in neuroticism & -0.0072 & -0.1977 & 0.1838 & 0.5143 \\ 
  g\_ij & 0.0141 & -0.1732 & 0.2033 & 0.4671 \\ 
  (1-g\_ij)*distance in classlist & -0.0665 & -0.1678 & 0.0241 & 0.8814 \\ 
   \hline \multicolumn{5}{c}{Utility (direct links)} \\ \hline intercept & -0.0157 & -0.1945 & 0.1811 & 0.5557 \\ 
  distance in age & 0.0029 & -0.1788 & 0.1861 & 0.4986 \\ 
  distance in gender & -0.012 & -0.2038 & 0.166 & 0.5371 \\ 
  distance in cognitive skills & -0.0062 & -0.187 & 0.1832 & 0.5129 \\ 
  distance in conscientiousness & -0.0075 & -0.1973 & 0.1711 & 0.53 \\ 
  distance in neuroticism & -0.0095 & -0.1915 & 0.1596 & 0.5114 \\ 
   \hline \multicolumn{5}{c}{Utility (reciprocal links)} \\ \hline intercept & 0.0012 & -0.1709 & 0.1725 & 0.4986 \\ 
  distance in age & 0.005 & -0.181 & 0.1871 & 0.4886 \\ 
  distance in gender & 0.0024 & -0.1744 & 0.1821 & 0.4857 \\ 
  distance in cognitive skills & 2e-04 & -0.1825 & 0.1876 & 0.4971 \\ 
  distance in conscientiousness & -8e-04 & -0.1784 & 0.1686 & 0.5029 \\ 
  distance in neuroticism & -0.0056 & -0.1875 & 0.1768 & 0.5243 \\ 
   \hline \multicolumn{5}{c}{Utility (indirect links)} \\ \hline intercept & -0.0756 & -0.226 & 0.0826 & 0.7843 \\ 
  distance in age & 0.0038 & -0.1187 & 0.1227 & 0.4729 \\ 
  distance in gender & -0.058 & -0.2248 & 0.1167 & 0.7129 \\ 
  distance in cognitive skills & -0.0072 & -0.189 & 0.1777 & 0.5386 \\ 
  distance in conscientiousness & -0.0502 & -0.2183 & 0.1011 & 0.6986 \\ 
  distance in neuroticism & -0.0478 & -0.2099 & 0.104 & 0.6843 \\ 
   \hline \multicolumn{5}{c}{Utility (popularity)} \\ \hline intercept & -0.0756 & -0.226 & 0.0826 & 0.7843 \\ 
  distance in age & 0.0038 & -0.119 & 0.1227 & 0.4729 \\ 
  distance in gender & -0.058 & -0.2249 & 0.1167 & 0.7129 \\ 
  distance in cognitive skills & -0.0072 & -0.1892 & 0.1777 & 0.5386 \\ 
  distance in conscientiousness & -0.0502 & -0.2183 & 0.1021 & 0.6986 \\ 
  distance in neuroticism & -0.0478 & -0.2095 & 0.104 & 0.6843 \\ 
   \hline
\hline
\label{results_unweighted_acceptance_0.01}
\end{longtable}


==> tables/results_proposal.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Jan 15 20:28:39 2020
\begin{longtable}{ccccc}
\label{results_proposal} \\
\caption{Posterior distribution. Unweighted criterion. Acceptance rate: 0.01. $\hat{\tau}_0 = 76$.} \\ 
  \hline
  & Mean & Q .05 & Q.95 & Prob $<$ 0 \\ 
  \hline \multicolumn{5}{c}{Matching parameters} \\ \hline
distance in age & 0.0478 & -0.0408 & 0.1318 & 0.1905 \\ 
  distance in gender & 0.0255 & -0.1054 & 0.1367 & 0.2582 \\ 
  distance in cognitive skills & 0.0255 & -0.0278 & 0.0768 & 0.1503 \\ 
  distance in conscientiousness & -0.0059 & -0.0785 & 0.0572 & 0.5703 \\ 
  distance in neuroticism & -0.0157 & -0.09 & 0.0629 & 0.6642 \\ 
  g\_ij & -0.0254 & -0.1049 & 0.0347 & 0.7685 \\ 
  (1-g\_ij)*distance in classlist & -0.0967 & -0.1532 & -0.0419 & 0.9993 \\ 
   \hline \multicolumn{5}{c}{Utility (direct links)} \\ \hline intercept & -0.0327 & -0.0826 & 0.016 & 0.8438 \\ 
  distance in age & -0.0908 & -0.1517 & -0.0367 & 0.9881 \\ 
  distance in gender & -0.0119 & -0.1222 & 0.0743 & 0.5988 \\ 
  distance in cognitive skills & -0.0118 & -0.092 & 0.0619 & 0.5328 \\ 
  distance in conscientiousness & -0.0256 & -0.0954 & 0.0475 & 0.6768 \\ 
  distance in neuroticism & -0.0254 & -0.0934 & 0.0452 & 0.6377 \\ 
   \hline \multicolumn{5}{c}{Utility (reciprocal links)} \\ \hline intercept & -0.0423 & -0.1073 & 0.0305 & 0.8452 \\ 
  distance in age & -0.0405 & -0.129 & 0.0506 & 0.6549 \\ 
  distance in gender & -0.0239 & -0.0892 & 0.0469 & 0.7553 \\ 
  distance in cognitive skills & -0.0651 & -0.119 & -0.0024 & 0.959 \\ 
  distance in conscientiousness & 0.0431 & 0.0012 & 0.0812 & 0.0413 \\ 
  distance in neuroticism & 0.0454 & -0.0148 & 0.0865 & 0.0835 \\ 
   \hline \multicolumn{5}{c}{Utility (indirect links)} \\ \hline intercept & -0.019 & -0.0628 & 0.0241 & 0.8317 \\ 
  distance in age & -0.0859 & -0.1589 & -0.0256 & 0.9943 \\ 
  distance in gender & -0.0145 & -0.0633 & 0.0405 & 0.6966 \\ 
  distance in cognitive skills & -0.0307 & -0.0958 & 0.0254 & 0.7346 \\ 
  distance in conscientiousness & -0.03 & -0.1013 & 0.0339 & 0.7906 \\ 
  distance in neuroticism & -0.0266 & -0.0776 & 0.0252 & 0.7876 \\ 
   \hline \multicolumn{5}{c}{Utility (popularity)} \\ \hline intercept & -0.019 & -0.0628 & 0.0241 & 0.8317 \\ 
  distance in age & -0.0859 & -0.1589 & -0.0256 & 0.9943 \\ 
  distance in gender & -0.0145 & -0.0633 & 0.0405 & 0.6966 \\ 
  distance in cognitive skills & -0.0307 & -0.0958 & 0.0254 & 0.7346 \\ 
  distance in conscientiousness & -0.03 & -0.1013 & 0.0339 & 0.7906 \\ 
  distance in neuroticism & -0.0266 & -0.0776 & 0.0252 & 0.7876 \\ 
   \hline
\hline
\label{results_unweighted_acceptance_0.01}
\end{longtable}


==> tables/summary_dyad.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sun, Jul 14, 2019 - 23:16:23
\begin{table}[H] \centering 
  \caption{Pairwise distance in covariates -- Summary statistics} 
  \label{tab_summary_dyad}
    \begin{adjustbox}{width = \textwidth}
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
edge (baseline) & 17,736 & 0.172 & 0.377 & 0 & 0 & 0 & 1 \\ 
edge (followup) & 17,736 & 0.179 & 0.383 & 0 & 0 & 0 & 1 \\ 
distance in classlist (baseline) & 17,736 & 8.009 & 5.553 & 1 & 3 & 12 & 30 \\ 
distance in age (years) (baseline) & 17,736 & 0.827 & 0.908 & 0.000 & 0.249 & 1.041 & 6.633 \\ 
distance in gender (baseline) & 17,736 & 0.502 & 0.500 & 0 & 0 & 1 & 1 \\ 
distance in cognitive skills (baseline)& 17,736 & 0.099 & 0.081 & 0.000 & 0.035 & 0.144 & 0.530 \\ 
distance in conscientiousness (baseline) & 17,736 & 0.568 & 0.485 & 0.000 & 0.207 & 0.798 & 3.275 \\ 
distance in neuroticism (baseline) & 17,736 & 0.676 & 0.538 & 0.000 & 0.249 & 0.976 & 3.491 \\ 
\hline \\[-1.8ex] 
\end{tabular}
\end{adjustbox}
\end{table} 

